Thesis: Tensor networks for dynamic spacetimes

Tensor networks give simple representations of complex quantum states. They have proven useful in the study of condensed matter systems and conformal fields, and recently have provided toy models of AdS/CFT. Underlying the tensor network - AdS/CFT connection is the association of a graph geometry with the tensor network. In the context of the AdS/CFT correspondence tensor network models have so far been limited to describing static spacetimes. In this thesis we look to extend tensor network models of AdS/CFT by describing the geometry of a dynamic spacetime using a tensor network. We provide a review of tensor networks in the context of AdS/CFT to motivate this extension, before proposing modifications of holographic tensor network models that capture features of AdS/CFT with dynamic spacetimes. This thesis includes the results of arXiv submission 1611.06220, along with a review of the relevant literature.

==> Makefile <==
          NAME1 = diss
       PRODUCT1 = $(NAME1).pdf
     TEXSOURCE1 = $(NAME1).tex \
		    abstract.tex ack.tex glossary.tex intro.tex \
		    ubcdiss.cls
           BBL1 = $(NAME1).bbl

#         NAME2 =
#      PRODUCT2 = $(NAME2).pdf
#    TEXSOURCE2 = $(NAME2).tex 
#          BBL2 = $(NAME2).bbl

      BIBINPUTS = biblio.bib

     PDFFIGURES = $(BUILTPDFFIGURES) ${PNGFIGURES}
     PNGFIGURES = 
     GIFFIGURES = 
     SVGFIGURES = 
# Following is for Berkeley Make syntax:
#BUILTPDFFIGURES = \
#		    ${PNGFIGURES:C/\.png/.pdf/g} \
#		    ${GIFFIGURES:C/\.gif/.pdf/g} \
#		    ${SVGFIGURES:C/\.svg/.pdf/g}

all: doc.pdf $(PRODUCT1)

$(NAME1).pdf: $(TEXSOURCE1) $(BBL1) $(PDFFIGURES)
$(NAME1).dvi: $(TEXSOURCE1) $(BBL1) $(EPSFIGURES)
$(NAME1).bbl: $(TEXSOURCE1) $(BIBINPUTS) $(PDFFIGURES)

#$(NAME2).pdf: $(TEXSOURCE2) $(BBL2) $(BUILTPDFFIGURES)
#$(NAME2).dvi: $(TEXSOURCE2) $(BBL2) $(BUILTEPSFIGURES)
#$(NAME2).bbl: $(TEXSOURCE2) $(BIBINPUTS) $(BUILTEPSFIGURES) $(BUILTPDFFIGURES)

clean:
	$(RM) ${BUILTPDFFIGURES} $(NAME1).aux $(NAME1).dvi \
	    $(NAME1).log $(NAME1).blg $(NAME1).bbl $(NAME1).out \
	    $(NAME1).toc $(NAME1).lof $(NAME1).lot $(NAME1).brf \
            *.aux

# configuration issues
.SUFFIXES: .tex .pdf .bbl

PDFLATEX=	pdflatex
BIBTEX=		bibtex
XELATEX=	xelatex 
LATEX=		latex
BIBLATEX=	$(PDFLATEX)
BIBTEX=		bibtex -min-crossref=1000
RM=		rm -f
MV=		mv
CP=		cp -p

.tex.pdf:
	$(PDFLATEX) $(LATEXFLAGS) $<
	@while egrep -q 'LaTeX Warning:.*Rerun|Rerun to get' $*.log; do \
	       echo $(PDFLATEX) $<; \
	      $(PDFLATEX) $(LATEXFLAGS) $< || exit $$?; \
	done

.tex.bbl: 
	$(BIBLATEX) $(LATEXFLAGS) $<
	$(BIBTEX) $*
	$(RM) $*.aux $*.dvi $*.pdf

doc.pdf: diss.pdf
	$(CP) diss.pdf doc.pdf


==> glossary.tex <==
%% The following is a directive for TeXShop to indicate the main file
%%!TEX root = diss.tex

\chapter{Glossary}

This glossary uses the handy \latexpackage{acroynym} package to automatically
maintain the glossary.  It uses the package's \texttt{printonlyused}
option to include only those acronyms explicitly referenced in the
\LaTeX\ source.

% use \acrodef to define an acronym, but no listing
\acrodef{UI}{user interface}
\acrodef{UBC}{University of British Columbia}

% The acronym environment will typeset only those acronyms that were
% *actually used* in the course of the document
\begin{acronym}[ANOVA]
\acro{ANOVA}[ANOVA]{Analysis of Variance\acroextra{, a set of
  statistical techniques to identify sources of variability between groups}}
\acro{API}{application programming interface}
\acro{CTAN}{\acroextra{The }Common \TeX\ Archive Network}
\acro{DOI}{Document Object Identifier\acroextra{ (see
    \url{http://doi.org})}}
\acro{GPS}[GPS]{Graduate and Postdoctoral Studies}
\acro{PDF}{Portable Document Format}
\acro{RCS}[RCS]{Revision control system\acroextra{, a software
    tool for tracking changes to a set of files}}
\acro{TLX}[TLX]{Task Load Index\acroextra{, an instrument for gauging
  the subjective mental workload experienced by a human in performing
  a task}}
\acro{UML}{Unified Modelling Language\acroextra{, a visual language
    for modelling the structure of software artefacts}}
\acro{URL}{Unique Resource Locator\acroextra{, used to describe a
    means for obtaining some resource on the world wide web}}
\acro{W3C}[W3C]{\acroextra{the }World Wide Web Consortium\acroextra{,
    the standards body for web technologies}}
\acro{XML}{Extensible Markup Language}
\end{acronym}

% You can also use \newacro{}{} to only define acronyms
% but without explictly creating a glossary
% 
% \newacro{ANOVA}[ANOVA]{Analysis of Variance\acroextra{, a set of
%   statistical techniques to identify sources of variability between groups.}}
% \newacro{API}[API]{application programming interface}
% \newacro{GOMS}[GOMS]{Goals, Operators, Methods, and Selection\acroextra{,
%   a framework for usability analysis.}}
% \newacro{TLX}[TLX]{Task Load Index\acroextra{, an instrument for gauging
%   the subjective mental workload experienced by a human in performing
%   a task.}}
% \newacro{UI}[UI]{user interface}
% \newacro{UML}[UML]{Unified Modelling Language}
% \newacro{W3C}[W3C]{World Wide Web Consortium}
% \newacro{XML}[XML]{Extensible Markup Language}

